Gluons and the quark sea at high energies: distributions, polarization, tomography

This report is based on a ten-week program on "Gluons and the quark sea at high-energies", which took place at the Institute for Nuclear Theory in Seattle in Fall 2010. The principal aim of the program was to develop and sharpen the science case for an Electron-Ion Collider (EIC), a facility that will be able to collide electrons and positrons with polarized protons and with light to heavy nuclei at high energies, offering unprecedented possibilities for in-depth studies of quantum chromodynamics. This report is organized around four major themes: i) the spin and flavor structure of the proton, ii) three-dimensional structure of nucleons and nuclei in momentum and configuration space, iii) QCD matter in nuclei, and iv) Electroweak physics and the search for physics beyond the Standard Model. Beginning with an executive summary, the report contains tables of key measurements, chapter overviews for each of the major scientific themes, and detailed individual contributions on various aspects of the scientific opportunities presented by an EIC.

==> Master/heavy.tex <==
\section{Theoretical Status of Inclusive Heavy Quark Production in Deep-Inelastic Scattering}
\label{sec:JB}


%%%%%%%%% insert author names addresses here, please do not change format

\hspace{\parindent}\parbox{\textwidth}{\slshape 
  Sergey Alekhin\,$^{1,2}$, Johannes Bl\"umlein\,$^1$ Sven-Olaf Moch\,$^1$ 
\\[1ex]
$^1$\ Deutsches Elektronen-Synchrotron, DESY, 
Platanenallee 6, D-15738 Zeuthen, Germany \\
$^2$\ 
Institute for High Energy Physics, 142281 Protvino, Moscow 
Region, Russia }

% put the author names here again, for the list of authors at the end of
% the volume
\index{Alekhin, Sergey}
\index{Bl\"umlein, Johannes}
\index{Moch, Sven-Olaf}

\vspace{2\baselineskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\centerline{\bf Abstract}
\vspace{0.7\baselineskip}
\parbox{0.9\textwidth}{A brief review of the theoretical
status of the inclusive heavy flavor
production in deep-inelastic scattering is given.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The heavy quark production gives a sizable contribution to the unpolarized 
DIS structure functions at small $x$~\cite{EXP}. For the foreseen EIC 
kinematics of deep-inelastic scattering (DIS) it yields up to 10\% of the inclusive 
cross section.
Therefore in order to employ the full 
potential of the small-$x$ EIC data for phenomenology 
one has to provide an accurate theoretical description of 
heavy-quark electro-production within perturbative QCD. 
In particular, this is necessary for a precise determination of 
$\alpha_s(M_Z^2)$ and the extraction of the parton distribution functions (PDFs) 
from the EIC data to be applied in
hadron collider physics~\cite{HLHC}. For the light-parton 
contribution the theoretical accuracy of $O$(few \%) is achieved, with 
the complete QCD corrections up to 3-loops available. In the case of 
the fixed-flavor-number scheme (FFNS) the heavy flavor corrections are available
only to $O(\alpha_s^2)$ in complete form.
This can be a bottleneck for the analysis of 
high-precision data. Therefore the progress in the higher-order 
calculations of 
heavy-quark-production coefficient functions is quite important for  
the EIC phenomenology. For the variable-flavor-number scheme (VFNS) the 
massive quarks are considered on the same footing as the massless ones. 
Furthermore, the heavy-quark PDFs appearing in the VFNS are derived 
from the light-parton PDFs with the massive operator-matrix elements (OMEs). 
The VFNS coefficient functions are known up to 3-loop 
accuracy due to the scheme definition. However, the massive OMEs are 
completely known up to the NLO corrections only and this limits 
the theoretical accuracy of the VFNS as well. 

In the following we summarize the state-of-art in calculations of 
the NNLO corrections to the unpolarized heavy-quark coefficient functions 
and to the massive OMEs.
Furthermore the FFNS and VFNS are compared to the available 
HERA data and to each other in the context of the high-order corrections. 
We also discuss the implementation of the running-mass scheme for 
the NLO and NNLO heavy-quark coefficient functions
and the resulting improvement in the perturbative stability related to this definition.
Finally, we give a brief review of available theoretical calculations 
for the polarized heavy-quark coefficient functions. 

\vspace*{-3mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Unpolarized structure functions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{General framework}

The heavy flavor corrections to deep-inelastic structure functions emerge in the
Wilson coefficients for the respective processes, i.e. they contribute
in terms of virtual and final state effects. Heavy quarks have no strict partonic 
interpretation since partons in the closer sense are massless, and by virtue of 
this, infinitely long lived, with the possibility to move collinear to each other.
Formally, they can form field-theoretic in- and out-states at $t = \mp \infty$.
Adopting this picture, heavy quarks can be singly or pair produced from other 
massless partons and the gauge bosons of the Standard Model as final states. This 
description
is called FFNS, which is the genuine scheme in any
quantum-field theoretic calculation. The structure functions $F_i(x,Q^2)$ obey the 
representation
%-----------------------------------------------------------------------------------
\begin{eqnarray}
F_i(x,Q^2) = \left[\sum_{k = q_l,g} \left[ 
C_{i,\sf light}^k(x,Q^2/\mu^2) +
C_{i,\sf heavy}^k(x,Q^2/\mu^2, m_h^2/\mu^2)\right] \otimes f^k(\mu^2)\right](x)~,
\end{eqnarray}
%-----------------------------------------------------------------------------------
where $q_l$ and $g$ label the massless quarks and gluons, $f^k(\mu^2)$ are the 
parton 
densities,
$C_{i,\sf light (heavy)}^k$ the massless resp. massive Wilson coefficients,
$\otimes$ denotes the Mellin convolution, and $h=c,b$ denote the 
$c$- and $b$-quarks. Other approaches derive from this description.

In case of unpolarized deep-inelastic scattering the leading order contributions
were given in \cite{LO} and the next-to-leading order (NLO) corrections were 
calculated in semi-analytic form  in \cite{NLO}. For asymptotic values $Q^2 \gg m_h^2$
one may obtain the massive Wilson coefficients in analytic form. This is due to a 
factorization theorem \cite{Buza:1995ie} of the massive Wilson coefficients into 
universal massive OMEs and the massless Wilson coefficients \cite{COEFF}
%-----------------------------------------------------------------------------------
\begin{eqnarray}
C_{i,\sf heavy}^l(x,Q^2/\mu^2, m_h^2/\mu^2) = \sum_k \left[A^{kl}(\mu^2/m_h^2) 
\otimes 
C_{i,k}(Q^2/\mu^2)\right](x)~.  
\end{eqnarray}
%-----------------------------------------------------------------------------------
As comparisons up to NLO showed \cite{Buza:1995ie} these representations are valid 
for the structure function $F_2(x,Q^2)$ if $Q^2/m_h^2 \gsim 10$.
To $O(\alpha_s^2)$ the Wilson coefficients were obtained in 
\cite{Buza:1995ie,TOL2,TOL2a} at general values of the Mellin variable $N$. A first 
contribution to the 3-loop corrections was given in \cite{Bierenbaum:2008yu} by the
$O(\alpha_s^2 \varepsilon)$ terms which contribute to the logarithmic terms
$O(\ln^k(Q^2/m_h^2)),~k = 1,2,3,$ in $O(\alpha_s^3)$. A large number of even 
Mellin-moments for all unpolarized 3-loop massive OMEs have 
been calculated in  \cite{Bierenbaum:2009mv} up to $N = 10 ... 14$ depending on the
respective channel. 
%In these calculations the code {\tt MATAD} 
%\cite{Steinhauser:2000ry} has 
%been extended to allow the computation of higher moments for local operator 
%insertions. As a by-product of this calculation the corresponding color 
%projections of the 3-loop anomalous dimensions have been obtained in agreement with
%earlier calculations \cite{ANOMD}. 
For the structure function $F_L(x,Q^2)$ the 
asymptotic 3-loop corrections were given in \cite{Blumlein:2006mh} for general 
values of $N$. However, they are valid at 1\% accuracy at much higher scales 
of $Q^2/m_h^2 \gsim 800$ only. All logarithmic terms at $O(\alpha_s^3)$ 
for the heavy flavor Wilson coefficients contributing to the structure function
$F_2(x,Q^2)$ are known \cite{LOG}. More than this, all the contributions  to the 
constant terms emerging from lower order contributions by renormalization have been 
calculated, cf.~\cite{Bierenbaum:2009mv} for details. At three loop order the five 
Wilson coefficients $H_{2,g}, H_{2,q}^{\sf PS}, 
L^{\sf NS}_q, L_{2,q}^{\sf PS}$, and
$L_{2,g}^{\sf S}$ contribute. In Ref.~\cite{Ablinger:2010ty} the latter two
Wilson coefficients have been calculated for general values of $N$ as well as the
terms $\propto T_F^2 n_f$, in the 
other cases, with $n_f$ the number of massless quark flavors. Due to the size of 
the constant 
contributions phenomenological applications for the kinematic range available at 
HERA cannot be based on only the logarithmic contributions. QCD corrections
to charged current heavy flavor production have been considered in \cite{CC}. 


\subsubsection{FFNS and VFNS}


The logarithmic contributions in the heavy flavor Wilson coefficients $\propto
\ln^k(Q^2/m_h^2)$ never become so large in the kinematic region of HERA that
their resummation 
would be required \cite{Gluck:1993dpa}. Nonetheless one may introduce 
a description changing the number of light flavors effectively, which
refers to the {\it universal} contributions to the 
heavy flavor Wilson coefficients,
consisting of the twist-2 parton densities and the massive OMEs
\cite{TOL2a,Bierenbaum:2009mv,Buza:1996wv,Collins:1998rz}. This requires the 
knowledge of also the gluonic OMEs 
$A_{gg}$ and $A_{gq}$ to 3-loop order 
\cite{Bierenbaum:2009mv}. 

\vspace*{-5mm}
\restylefloat{figure}
\begin{center}
\begin{figure}[H] %%[b]
\epsfig{figure=BMSN.eps,width=\linewidth} 

\vspace*{-1mm}
\caption[]{
\label{FIG1}
\small 
Comparison of $F^c_2$
in different schemes to H1- and ZEUS-data. Solid lines: GMVFNS
in the BMSN prescription, dash-dotted lines: 3-flavor scheme, dashed lines: 
4-flavor scheme. The vertical
dotted line denotes the position of the charm-quark mass $m_c$ = 1.43~GeV, from 
Ref.~\cite{Alekhin:2009ni}.}
\end{figure}
\end{center}

\vspace*{-1.1cm}
By matching at typical scales $\mu_f$ one performs 
the transition from $n_f$ to $n_f+1$ massless flavors using asymptotic relations.
In this way one may introduce a heavy quark density at the expense of all other 
flavor densities being massless. The corresponding representation which is obtained
in terms of a reformulation of the FFNS is called zero mass variable flavor number
scheme (ZMVFNS) and is unique up to the choice of the matching point(s). 
An important issue is the choice of the scale $\mu_f$, for which very often $\mu_f 
\simeq m_{h}$ is used. In Ref.~\cite{Blumlein:1998sh} it was shown, however, 
comparing exact and flavor number matched calculations that this scale is process 
dependent and frequently very different scales have to be chosen. In this 
context various problems are arising. Because of the value of
the charm to bottom mass ratio, 
$m_c^2/m_b^2 \sim 1/9$, power corrections due to 
$m_c^2$ can normally 
not be neglected at scales $\mu^2 \simeq m_b^2$. Therefore, sequential decoupling 
of both charm and bottom quarks is problematic. Furthermore, starting with  
$O(\alpha_s^3)$ Feynman diagrams with both bottom- and charm-quarks contribute, 
which cannot be attributed to either the charm or the bottom quark density 
\cite{Blumlein:2010yc}. The description of the FFNS, on the other hand, is still 
possible. Therefore representations based on the ZMVFNS remain approximations
to which one may refer for specific applications. 
Furthermore, it applies for the asymptotic case $Q^2 \gg m_h^2$.
Meanwhile for the description of realistic data
%the heavy flavor contributions to the structure function $F_2(x,Q^2)$ 
one would 
like to have a smooth description of the structure functions both at large 
and low $Q^2$, which is called general mass variable flavor number scheme 
(GMVFNS). 
%The current implementation of the
%heavy flavor corrections for the structure function $F_2(x,Q^2)$ is performed at $O(\alpha_s^2)$.
Here an important smooth interpolation is 
provided by the BMSN scheme~\cite{Buza:1996wv,Alekhin:2009ni} given by
%-----------------------------------------------------------------------------------
\begin{eqnarray}
\label{eq3}
F_2^{h,\sf BMSN}(n_f+1) = 
F_2^{h,\sf exact}(n_f)
+ F_2^{h,\sf ZMFVN}(n_f+1)
- F_2^{h,\sf asymp}(n_f)~,
\end{eqnarray}
%-----------------------------------------------------------------------------------
where {\sf exact} corresponds to \cite{NLO}, {\sf asymp} its asymptotic form for
$Q^2 \gg m_h^2$.
%, and {\sf ZMVFNS} to the value in the zero mass variable flavor scheme.
In Figure~\ref{FIG1} this transition is shown for values of $x$ between 0.0002 and 
0.013 for the kinematics at HERA according to (\ref{eq3}) 
(see Ref.~\cite{Ajaltouni:2009zz} for phenomenological variants
of the GMVFNS). 




\vspace*{-3mm}
\subsubsection{The massive NNLO corrections and the running mass}


The radiative corrections to the massive Wilson coefficients are known to be sizable. 
In particular near the production threshold $s \simeq 4 m_h^2$ 
where large Sudakov double logarithms dominate at each order $\alpha_s^k ln^{2k}(1 - 4m_h^2/s)$ 
one may apply resummations
starting with the fully differential 1-loop cross section through which 
dominant parts of the higher order corrections in the coupling constant are covered. These
contributions have been given in Refs.~\cite{THRESH} in detail. 

\vspace*{-3mm}
\noindent
%\usepackage{float}
\restylefloat{figure}
\begin{center}
\begin{figure}[H] %%[b]
\epsfig{figure=plot-pole-cen.eps,width=0.48\linewidth} \hspace*{2mm}
\epsfig{figure=plot-msbar-cen.eps,width=0.48\linewidth}
\caption[]{
\label{FIG3}
\small 
The mass dependence of the NC charm structure function $F^p_2$
for a proton with $Q^2$ = 10~GeV$^2$,
$x = 10^{-3}$ and $\mu_r = \mu_f = \sqrt{Q^2 +4 m^2_c}$
using the PDFs \cite{Alekhin:2009ni}. The charm-quark mass is taken in the on-shell
scheme (left) and in the MSscheme (right) at LO (blue), NLO (green) and NNLOapprox 
(red); from Ref.~\cite{Alekhin:2010sv}.}
\end{figure}
\end{center}

\vspace*{-5mm}
\restylefloat{figure}
\begin{center}
\begin{figure}[H] %%[b]
\epsfig{figure=f2c_vs_abkm_running_mc.eps,width=\linewidth,height=11cm} 

\vspace*{-1mm}
\caption[]{
\label{FIG5}
\small 
The combined HERA data on the semi-inclusive structure function $F_2^{cc}$ 
in comparison with the prediction of fit~\cite{Alekhin:2010sv} performed in 
the running-mass scheme~\cite{Lipka}.}
\end{figure}
\end{center}



Another aspect at higher orders concerns the definition of the heavy quark mass, 
since it is a scheme dependent quantity.
It is of particular interest to investigate which
choice of scheme leads to a faster convergence of the perturbative series. 
Upon conversion of the conventionally used on-shell mass for heavy quark DIS to the
running mass $m_h(\mu)$ in the $\overline{\rm MS}$-scheme one observes considerable
improvement of scale stability and convergence of the perturbative expansion.
The latter aspect is demonstrated in Figure~\ref{FIG3}. Here
one uses the Wilson coefficients to NLO and refers to the approximate result
valid in the threshold region~\cite{THRESH} to give an estimate for the NNLO value,
see Ref.~\cite{Alekhin:2010sv}. As demonstrated in Figure~\ref{FIG3}, in case of the 
definition of the heavy quark mass in the $\overline{\rm MS}$ scheme the 
convergence is faster than in the on-mass shell scheme.  

The phenomenological impact of the mass scheme re-definition was checked on the 
example 
of ABKM fit of Ref.~\cite{Alekhin:2009ni}. In the variant of this fit~\cite{Alekhin:2010sv}
the heavy-quark electro-production was considered in the running mass scheme and 
with the approximate NNLO corrections taken into account.    
The $c$-quark mass was fitted to the DIS data simultaneously 
with the PDF parameters with the $c$-quark mass world average provided by 
PDG~\cite{Nakamura:2010zzi} 
added to the fit as an additional constraint. In this way the value of 
$m_c(m_c)=1.18\pm0.06~{\rm GeV}$ was obtained. The predictions for semi-inclusive 
structure function $F_2^{c\overline{c}}$ calculated in the running-mass scheme with 
this value 
of $m_c$ and the PDFs of Ref.~\cite{Alekhin:2010sv} are in good agreement with the 
preliminary HERA data on $F_2^{c\overline{c}}$ in a wide kinematical region, cf. 
Figure~\ref{FIG5}. This comparison gives an additional justification of the 
FFNS validity up to $Q^2\sim 1000~{\rm GeV}^2$.  


\vspace*{-0.7cm}
\noindent

\vspace{-5mm}
\restylefloat{figure}
\begin{center}
\begin{figure}[h] %%[b]
\epsfig{figure=ABKM09.eps,width=\linewidth}
\vspace*{-5mm}
\caption[]{
\label{FIG2}
\small 
The 1$\sigma$ error bands (shaded area) for our NNLO 4-flavor (left panel) and 
5-flavor (central
and right panels) $s$-, $c$-, and $b$-quark distributions in comparison to the 
corresponding MSTW2008 NNLO
distributions \cite{Martin:2009iq} (dashed lines); from 
Ref.~\cite{Alekhin:2009ni}.}
\end{figure}
\end{center}

\vspace*{-5mm}
\noindent


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Heavy-flavor PDFs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let us now discuss some phenomenological aspects. 
For applications at high-energy hadron colliders, schemes with 4- and 5-light
flavors need to be considered. The necessary charm- and bottom PDFs are
generated perturbatively.
In Figure~\ref{FIG2} the results for the NNLO parton densities for the heavier flavors $s,c$ 
and $b$ are shown, determined in two fits to the world data 
\cite{Alekhin:2009ni,Martin:2009iq}. The 1$\sigma$ error bands correspond to the 
analysis \cite{Alekhin:2009ni}. The central value of the MSTW08 distributions 
turn out to lie below  
those found in the ABKM09 analysis for the $c$ and $b$ quark distributions in the 
whole kinematic range at HERA, which results from the lower gluon density 
\cite{Martin:2009iq}. 
The strange quark distribution still exhibits large errors. Closer agreement was 
found
comparing between the parton densities of ABKM09 and JR 
\cite{JimenezDelgado:2008hf},
see Ref.~\cite{Alekhin:2009ni}. 
Updates of the ABKM09 distribution \cite{Alekhin:2010iu} lead to slight 
modifications of the heavy quark densities. We also remark that there is a small 
contribution due to heavy flavor within the flavor non-singlet analyses 
starting at $O(\alpha_s^2)$ \cite{NSI}.  Measurements at the EIC can 
both considerably improve the strange and charm quark densities in runs at highest 
luminosity. 



\subsection{Polarized structure functions}

For polarized deep-inelastic scattering the leading order corrections were given in
\cite{PLO}. The NLO corrections are known only in the asymptotic case $Q^2 \gg m_h^2$ 
\cite{PNLO}. In the flavor non-singlet case the 3-loop moments up to $N=13$
were given in \cite{Bierenbaum:2009mv}. In Ref. \cite{Ablinger:2010ty} also the
$O(\alpha_s T_F^2 n_f)$ contributions to the non-singlet OMEs 
and to transversity at general values of $N$ are given. For the gluonic 
heavy flavor corrections at 
twist 2 to the  structure function $g_2(x,Q^2)$ it has been shown that it can be 
obtained through a Wandzura-Wilczek relation \cite{Blumlein:2003wk} to all orders. 
The leading order threshold resummation of the 1-loop Wilson coefficient has been 
performed in \cite{Eynck:2000gz}. Finally, heavy flavor contributions at the 2- and 
3-loop level have been computed to transversity in the asymptotic region in 
\cite{Blumlein:2009rg}.

\vspace*{-12mm}
%\usepackage{float}
\restylefloat{figure}
\begin{center}
\begin{figure}[H] %%[b]
\epsfig{figure=g1ccbar.eps,width=0.48\linewidth} \hspace*{2mm}
\epsfig{figure=g2ccbar.eps,width=0.48\linewidth}

\vspace*{-1mm}
\caption[]{
\label{FIG4}
\small 
Heavy flavor contributions to the polarized structure
function $xg_1(x,Q^2)$ using the leading order parameterization ISET=1 of
\cite{Bluemlein:2002be}, ($\Lambda_{\rm QCD} = 203$ MeV) 
as a function of $x$ and $Q^2$. Upper lines: $g_{1}^{cc}(x,Q^2)$ for $m_c = 1.5$ 
GeV. Full line, $Q^2 = 4$ GeV$^2$; dashed line,
$Q^2=10$ GeV$^2$; dotted line, $Q^2$ = 100 GeV$^2$; dash-dotted line, $Q^2
 = 1000$ GeV$^2$. Lower lines: $g_1^{cc}(x,Q^2)$ for $m_b = 4.3$ GeV. Dotted
line, $Q^2 = 100$ GeV$^2$; dash-dotted line, $Q^2 =1000$ GeV$^2$. (b) Heavy
flavor contributions to the polarized structure function $xg_2(x,Q^2)$.
All conditions are the same as in (a); from Ref.~\cite{Blumlein:2003wk}.
}
\end{figure}
\end{center}

\vspace*{-7mm}
\noindent

In the polarized case the heavy quark contributions to the structure functions
$g_{1,2}(x,Q^2)$ are comparably smaller than in the unpolarized case, which is both
a consequence of the relative size of the polarized gluon distribution function 
to the other polarized parton densities and because of a sum rule for the first 
moment of the gluonic Wilson coefficient for $g_{1}(x,Q^2)$. In addition, there is 
a Wandzura-Wilczek relation for the gluonic contribution to $g_{2}(x,Q^2)$, 
cf.~\cite{Blumlein:2003wk}. In Ref.~\cite{Blumlein:2010rn} the 
$O(\alpha_s)$ deep-inelastic heavy flavor 
Wilson coefficient was taken into account in an inclusive world
data analysis. Figure~\ref{FIG4} illustrates the charm contributions to $g_{1,2}(x,Q^2)$
in a wide kinematic range. Their measurement is one of the challenges at the 
EIC. Due to the specific structure of these distributions it also provides 
interesting QCD tests in a twofold sense: {\it i)} the corresponding form of the 
Wilson coefficients can be verified. {\it ii)} The lines in Figure~\ref{FIG4} were 
calculated for a positive polarized gluon density $\Delta G$. The oscillation
reverses in case of a negative gluon density and will look rather different in 
the case that
$\Delta G$ changes sign within the $x$-range probed.

In conclusion, high luminosity measurements of the heavy flavor contributions to 
the unpolarized and polarized deep-inelastic structure functions will deliver a
much more refined picture of the nucleon sub-structure than the one available now, 
bearing
experimental challenges which will significantly deepen the physical understanding
of these structures.    
%-----------------------------------------------------------------------------
\begin{thebibliography}{99}
%-----------------------------------------------------------------------------
%
%[2]
\bibitem{EXP}
%-----------------
%\cite{Aaron:2010ib}
%\bibitem{Aaron:2010ib}
  F.~D.~Aaron {\it et al.}  [H1 Collaboration],
  %``Measurement of Charm and Beauty Jets in Deep Inelastic Scattering at
  %HERA,''
  arXiv:1008.1731 [hep-ex];
  %%CITATION = ARXIV:1008.1731;%%
%-----------------
%\cite{:2009ut}
%\bibitem{:2009ut}
%  F.~D.~Aaron {\it et al.}  [H1 Collaboration],
  %``Measurement of the Charm and Beauty Structure Functions using the H1 Vertex
  %Detector at HERA,''
  Eur.\ Phys.\ J.\   {\bf C65}, 89 (2010),
  [arXiv:0907.2643 [hep-ex]];\\
  %%CITATION = EPHJA,C65,89;%%
%-----------------
%\cite{Aktas:2006vs}
%\bibitem{Aktas:2006vs}
  A.~Aktas {\it et al.}  [H1 Collaboration],
  %``Measurement of charm and beauty dijet cross sections in photoproduction  at
  %HERA using the H1 vertex detector,''
  Eur.\ Phys.\ J.\   {\bf C47}, 597 (2006),
  [arXiv:hep-ex/0605016];
  %%CITATION = EPHJA,C47,597;%%
%-----------------
%\cite{Aktas:2005zc}
%\bibitem{Aktas:2005zc}
%  A.~Aktas {\it et al.}  [H1 Collaboration],
  %``Measurement of beauty production at HERA using events with muons and
  %jets,''
  Eur.\ Phys.\ J.\   {\bf C41}, 453 (2005),
  [arXiv:hep-ex/0502010];\\
  %%CITATION = EPHJA,C41,453;%%
%-----------------
%\cite{Chekanov:2009kj}
%\bibitem{Chekanov:2009kj}
  S.~Chekanov {\it et al.}  [ZEUS Collaboration],
  %``Measurement of charm and beauty production in deep inelastic ep scattering
  %from decays into muons at HERA,''
  Eur.\ Phys.\ J.\   {\bf C65}, 65 (2010),
  [arXiv:0904.3487 [hep-ex]];
  %%CITATION = EPHJA,C65,65;%%
%-----------------
%\cite{Chekanov:2008zz}
%\bibitem{Chekanov:2008zz}
%  S.~Chekanov {\it et al.}  [ZEUS Collaboration],
  %``Measurement of beauty production from dimuon events at HERA,''
  JHEP {\bf 0902}, 032 (2009),
  [arXiv:0811.0894 [hep-ex]].
  %%CITATION = JHEPA,0902,032;%%
%-----------------
%\cite{Chekanov:2004tk}
%\bibitem{Chekanov:2004tk}
%  S.~Chekanov {\it et al.}  [ZEUS Collaboration],
  %``Measurement of beauty production in deep inelastic scattering at HERA,''
  Phys.\ Lett.\   {\bf B599}, 173  (2004), 
  [arXiv:hep-ex/0405069];\\
  %%CITATION = PHLTA,B599,173;%%
%-----------------
%\cite{Abramowicz:2010zq}
%\bibitem{Abramowicz:2010zq}
  H.~Abramowicz {\it et al.}  [ZEUS collaboration],
  %``Measurement of beauty production in DIS and F_2^bbbar extraction at ZEUS,''
  arXiv:1005.3396 [hep-ex].
  %%CITATION = ARXIV:1005.3396;%%
%----------------------------------------------------------------------------------- 
%
%-----------------------------------------------------------------------------
%
%[1]
\bibitem{HLHC}
%\cite{Dittmar:2005ed}
%\bibitem{Dittmar:2005ed}
  M.~Dittmar, S.~Forte, A.~Glazov {\it et al.},
  %``Working Group I: Parton distributions: Summary report for the HERA LHC Workshop Proceedings,''
  [hep-ph/0511119];\\
%\cite{Alekhin:2005dx}
%\bibitem{Alekhin:2005dx}
  S.~Alekhin, G.~Altarelli, N.~Amapane {\it et al.},
  %``HERA and the LHC: A Workshop on the implications of HERA for LHC physics: Proceedings Part A,''
  [hep-ph/0601012],[hep-ph/0601013];\\
%\cite{Jung:2009eq}
%\bibitem{Jung:2009eq}
  Z.~J.~Ajaltouni, S.~Albino, G.~Altarelli {\it et al.},
  %``Proceedings of the workshop: HERA and the LHC workshop series on the implications of HERA for LHC physics,''
  [arXiv:0903.3861 [hep-ph]];\\
%\cite{Alekhin:2010dd}
%\bibitem{Alekhin:2010dd}
  S.~Alekhin, J.~Bl\"umlein, P.~Jimenez-Delgado, S.~Moch and E.~Reya,
  %``NNLO Benchmarks for Gauge and Higgs Boson Production at TeV Hadron
  %Colliders,''
  Phys.\ Lett.\  {\bf B697}, 127 (2011)
  [arXiv:1011.6259 [hep-ph]].
  %%CITATION = PHLTA,B697,127;%%
%[3]
\bibitem{LO}
%\cite{Witten:1975bh}
%\bibitem{Witten:1975bh}
  E.~Witten,
  %``Heavy Quark Contributions to Deep Inelastic Scattering,''
  Nucl.\ Phys.\  {\bf B104}, 445 (1976);\\
%\cite{Babcock:1977fi}
%\bibitem{Babcock:1977fi}
  J.~Babcock, D.~W.~Sivers, S.~Wolfram,
  %``QCD Estimates for Heavy Particle Production,''
  Phys.\ Rev.\  {\bf D18}, 162 (1978);\\
%\cite{Novikov:1977yc}
%\bibitem{Novikov:1977yc}
  V.~A.~Novikov, M.~A.~Shifman, A.~I.~Vainshtein, V.~I.~Zakharov,
  %``Charm Photoproduction and Quantum Chromodynamics,''
  Nucl.\ Phys.\  {\bf B136}, 125 (1978);\\
%\cite{Leveille:1978px}
%\bibitem{Leveille:1978px}
  J.~P.~Leveille, T.~J.~Weiler,
  %``Characteristics of Heavy Quark Leptoproduction in QCD,''
  Nucl.\ Phys.\  {\bf B147}, 147 (1979).
%-----------------------------------------------------------------------------
%
%[4]
\bibitem{NLO}
%\cite{Laenen:1992zk}
%\bibitem{Laenen:1992zk}
  E.~Laenen, S.~Riemersma, J.~Smith, W.L. van Neerven,
  %``Complete O (alpha-s) corrections to heavy flavor structure functions in electroproduction,''
  Nucl.\ Phys.\  {\bf B392 }, 162, 229  (1993); \\
%\cite{Laenen:1992xs}
%\bibitem{Laenen:1992xs}
%  E.~Laenen, S.~Riemersma, J.~Smith {\it et al.},
%  %``O(alpha-s) corrections to heavy flavor inclusive distributions in 
%electroproduction,''
%  Nucl.\ Phys.\  {\bf B392 } (1993)  
%229.\\
%\cite{Riemersma:1994hv}
%\bibitem{Riemersma:1994hv}
  S.~Riemersma, J.~Smith, W.~L.~van Neerven,
  %``Rates for inclusive deep inelastic electroproduction of charm quarks at HERA,''
  Phys.\ Lett.\  {\bf B347 } 143 (1995),
  [hep-ph/9411431];\\
%\cite{Alekhin:2003ev}
%\bibitem{Alekhin:2003ev}
  Precise representations in Mellin space were derived in~:
  S.~I.~Alekhin and J.~Bl\"umlein,
  %``Mellin representation for the heavy flavor contributions to deep  inelastic
  %structure functions,''
  Phys.\ Lett.\   {\bf B594}, 299 (2004),
  [arXiv:hep-ph/0404034].
  %%CITATION = PHLTA,B594,299;%%
%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------
% 
%[6] 
\bibitem{COEFF}
%\cite{Furmanski:1981cw}
%\bibitem{Furmanski:1981cw}
  W.~Furmanski, R.~Petronzio,
  %``Lepton - Hadron Processes Beyond Leading Order in Quantum Chromodynamics,''
  Z.\ Phys.\  {\bf C11}, 293 (1982) and references therein;\\
%\cite{vanNeerven:1991nn}
%\bibitem{vanNeerven:1991nn}
  W.~L.~van Neerven, E.~B.~Zijlstra,
  %``Order alpha-s**2 contributions to the deep inelastic Wilson coefficient,''
  Phys.\ Lett.\  {\bf B272}, 127 (1991);
%\cite{Zijlstra:1991qc}
%\bibitem{Zijlstra:1991qc}
%  E.~B.~Zijlstra, W.~L.~van Neerven,
%  %``Contribution of the second order gluonic Wilson coefficient to the deep inelastic structure function,''
%  Phys.\ Lett.\  
{\bf B273}, 476 (1991);
%\cite{vanNeerven:1991gh}
%\bibitem{vanNeerven:1991gh}
%  W.~L.~van Neerven, E.~B.~Zijlstra,
  %``The O (alpha-s**2) corrected Drell-Yan K factor in the DIS and MS scheme,''
  Nucl.\ Phys.\  {\bf B382}, 11 (1992);\\
%\cite{Vermaseren:2005qc}
%\bibitem{Vermaseren:2005qc}
  J.~A.~M.~Vermaseren, A.~Vogt and S.~Moch,
  %``The third-order QCD corrections to deep-inelastic scattering by photon
  %exchange,''
  Nucl.\ Phys.\   {\bf B724}, 3 (2005),
  [hep-ph/0504242].
  %%CITATION = NUPHA,B724,3;%%
%-----------------------------------------------------------------------------------
%
%[7]
\bibitem{TOL2}
%\cite{Bierenbaum:2007qe}
%\bibitem{Bierenbaum:2007qe}
  I.~Bierenbaum, J.~Bl\"umlein and S.~Klein,
  %``Two-loop massive operator matrix elements and unpolarized heavy flavor
  %production at asymptotic values Q**2 >> m**2,''
  Nucl.\ Phys.\ {\bf B780}, 40  (2007),
  [hep-ph/0703285];
  %%CITATION = NUPHA,B780,40;%%
%\cite{Bierenbaum:2007dm}
%\bibitem{Bierenbaum:2007dm}
%  I.~Bierenbaum, J.~Bl\"umlein and S.~Klein,
  %``Calculation of massive 2-loop operator matrix elements with outer gluon
  %lines,''
  Phys.\ Lett.\ {\bf B648}, 195 (2007),
   [hep-ph/0702265];  
  %%CITATION = PHLTA,B648,195;%%
%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------
%
%[14]
\bibitem{LOG}
%\cite{Bierenbaum:2010jp}
%\bibitem{Bierenbaum:2010jp}
  I.~Bierenbaum, J.~Bl\"umlein and S.~Klein,
  %``Logarithmic $O(\alpha_s^3)$ contributions to the DIS Heavy Flavor Wilson
  %Coefficients at $Q^2 \gg m^2$,''
  arXiv:1008.0792 [hep-ph]; \\
  %%CITATION = ARXIV:1008.0792;%%
J. Ablinger, I.~Bierenbaum, J.~Bl\"umlein, S.~Klein, and F. Wi\ss{}brock, in 
preparation.
%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------
%
%[16]
\bibitem{CC}
%\cite{Gluck:1996ve}
%\bibitem{Gluck:1996ve}
  M.~Gl\"uck, S.~Kretzer, E.~Reya,
  %``The Strange sea density and charm production in deep inelastic charged current processes,''
  Phys.\ Lett.\  {\bf B380}, 171 (1996),
  [hep-ph/9603304]; \\
%\cite{Buza:1997mg}
%\bibitem{Buza:1997mg}
  M.~Buza, W.~L.~van Neerven,
  %``O (alpha-s**2) contributions to charm production in charged current deep inelastic lepton - hadron scattering,''
  Nucl.\ Phys.\  {\bf B500}, 301 (1997).
  [hep-ph/9702242];\\
  J. Bl\"umlein, A. Hasselhuhn, P. Kovacikova, and S.-O. Moch, DESY 11--032.
%-----------------------------------------------------------------------------



\bibitem{Lipka}
 K.Lipka, private communication. 

%-----------------------------------------------------------------------------
%-----------------------------------------------------------------------------

%-----------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------

%----------------------------------------------------------------------------------- 
\end{thebibliography}
\end{document}

